Physics Informed Data Driven model for Flood Prediction: Application of Deep Learning in prediction of urban flood development

Flash floods in urban areas occur with increasing frequency. Detecting these floods would greatlyhelp alleviate human and economic losses. However, current flood prediction methods are eithertoo slow or too simplified to capture the flood development in details. Using Deep Neural Networks,this work aims at boosting the computational speed of a physics-based 2-D urban flood predictionmethod, governed by the Shallow Water Equation (SWE). Convolutional Neural Networks(CNN)and conditional Generative Adversarial Neural Networks(cGANs) are applied to extract the dy-namics of flood from the data simulated by a Partial Differential Equation(PDE) solver. Theperformance of the data-driven model is evaluated in terms of Mean Squared Error(MSE) andPeak Signal to Noise Ratio(PSNR). The deep learning-based, data-driven flood prediction modelis shown to be able to provide precise real-time predictions of flood development

==> tex/2_Relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

% Literature review will make up of papers from three aspects. 
% \begin{itemize}
%     \item paper about flood prediction
%     \item paper about method used in simulation of shallow water equation
%     \item paper about using deep learning to learn PDE 
% \end{itemize}
% In this section, we briefly summarize the state of the art in related fields. Several fields are related to this topic. We first discuss presently used flood prediction methods. We next introduce new advances in solving PDE problem with deep learning techniques.

\subsection{Shallow Water Equation}
\kun{Shallow Water Equation(SWE), with its origin in the Navier-Stokes Equation, is widely applied to environmental flow simulation. The general characteristic of shallow water flows is that the vertical dimension is much smaller than the horizontal scale. Although SWE shows a 3-D characteristic because of the bottom friction \cite{vreugdenhil2013numerical},  in most cases, it's sufficient to average over the vertical horizon to get the 2-D SWE. 

The study of SWE can be traced back to very early when Laplace studied the tide. In 1-D case, SWE is also called Saint-Venant Equation \cite{dronkers1964tidal} which is usually used to simulate flow in river channels. In this work, 2-D SWE is focused on. Early works on SWE applied it in simulation of tidal \cite{riderinkhof1990residual}, atmospheric flows\cite{charney1950numerical} and storm surges\cite{dube1985numerical} etc.. Since \cite{alcrudo1993high}, finite volume method is popular for the numerical simulation of SWE. \cite{anastasiou1997solution} extended the finite volume based numerical solution of SWE to unstructured mesh. \cite{kurganov2002central, audusse2004fast, kurganov2007second, liang2009numerical} contributes to the 'well-balanced' numerical simulation of SWE which can preserve the dry area and still water. People also studied the well-balanced solution to wet-dry front problem in SWE\cite{horvath2015two, bollermann2013well}.
Recent researches also probe into implementing SWE numerical simulation on Graphics Processing Units(GPU)\cite{brodtkorb2012efficient}.}

\subsection{Flood prediction and Flood monitoring}

\textbf{Flood Prediction}

The research into prediction of flood hazards can be divided into two two kinds. Physics informed model prediction and Statistics based flood prediction. 

For physics based prediction models, a Partial Differential Equation (PDE) based model is used to predict the evolution of floods. SWE has been applied to many fields including storms\cite{borah2011hydrologic, costabile2013storm}, rainfall/runoff\cite{cea2010experimental, fernandez2016rainfall} and floods\cite{xia2017efficient}. Systematic error in parameter selection of PDEs can cause the fail of physics based methods\cite{mosavi2018flood}. More recent works including  \cite{bellos2016hybrid, bout2018validity}  brings improvements to the drawbacks with advanced flow simulation methods and hybrid models. However, the huge computational amount still obstructs these PDE based methods to be applied to real-time prediction task \cite{nayak2005short}. 

% \In the early ages, \cite{yakowitz1985markov} formulated the flood warning problem into a Markov Process to predict flood warning with current and previous status.

Instead of using hydrological flood propagation models, some researchers instead solely rely on historical data to predict future flood/tide events. These statistical techniques rely on the historical data and time series regression techniques\cite{khac2012data, damle2007flood, xiong2001non, laio2003comparison, valipour2012parameters, valipour2013comparison, basha2008model}. Since these methods require a large amount of historical data, they are usually applied to only river basins where fixed gauge station is installed. Besides, only a general prediction can be made, over a limited geographical area around the sensor\cite{mosavi2018flood}. 
% In history data based flood prediction, people combine machine learning techniques and history data to forecast flood in a river basin[\cite{khac2012data}]. \cite{damle2007flood} studied an application of time space data mining method to predict the river pattern with data from Mississippi River, St Louis gauging station.  

Interested readers can refer to \cite{mosavi2018flood} for a detailed review for the application of machine learning techniques to flood predictions. This section would focus on the application of neural networks related techniques in flood predicting.

Most researchers apply Neural Networks to draw data-driven model from historical monitoring data of river \cite{elsafi2014artificial} and areas prone to flood \cite{coulibaly2000daily, sattari2012performance}. \cite{chen2013reinforced} proposed a way to dynamically update the parameters in the prediction framework in an online learning style with Recurrent Neural Network. \cite{humphrey2016hybrid} proposed an Bayesian Neural Network based method to predict monthly stream flow changes. Similar techniques are applied to rainfall/runoff prediction \cite{smith1995neural} and precipitation prediction \cite{hassan2015suitability}. \cite{chen2015comparative} did a comparative study of the application of different optimization methods to river stream prediction in which hybrid neural network is mentioned.

% The issue of this kind of prediction method is that it is only suitable for the prediction of large scale area of flood conditions. Also the time resolution is usually in the scale of days. Thus, we can hardly apply it to the real-time flood estimation of urban area as we require the updates of precise flood distribution information around the city wide at the time step of at most every $30$ minutes.

The proposed work differs from existing contributions as follows. First, in contrast to current works mainly focus on statistics based prediction methods, this works relies on the physics-based prediction model which can be applied to areas that short in history flood data. Secondly, comparing to traditional physics based prediction models, the Deep Learning based data-driven model can predict in real-time, while preserving the accuracy of the prediction. Thirdly, in contrast to simplified computation models\cite{moore1994rffs}, the model in this work can give a precise and detailed prediction of the whole studied area. 

\textbf{Data Assimilation and Flood Prediction}

Starting from \cite{kalman1960new}, modern estimation techniques have been based on Bayesian Tracking, to conduct prior update and  posterior update steps. Extended Kalman filters, Unscented Kalman filters~\cite{wan2000unscented} and Particle filters\cite{arulampalam2002tutorial} are widely used in estimation of large scale nonlinear and distributed systems. 

In the field of flood estimation, \cite{georgakakos1986generalized} developed a flood prediction model and introduced the estimation method using Extended Kalman Filter. Earlier, \cite{yakowitz1985markov} formulated the flood warning problem into a Markov Process to predict flood warnings using current and previous states. \cite{basha2008model} presents an early flood warning system based on neural network for decision making.

In contrast with earlier works, the physics informed flood prediction method developed in this article provides a possibility to let people conduct a detailed, precise and real time estimation of the flood evolution over a large scale urban area with any Bayesian Tracking based estimation method.

\subsection{Deep Learning and Partial Differential Equations}
People in the PDE community have applied deep learning based methods to solve other PDE related problems. Their work can be broadly divided into two classes. 

In the first class, an exact solution to PDE which is represented partly or totally by Deep Neural network is given. This kind of method usually depends on neural network to explore a suitable combination of basis functions to form an exact solution to PDEs. Automatic differentiation technique helps in this procedure. The problem can be generally formulated into an optimization problem to minimize the gap between values evaluated at certain areas of the learned function and the observed data \cite{raissi2018deep, raissi2017physics1, raissi2017physics2}. \cite{long2017pde} combined Neural Network with specifically designed filters to uncover the dynamics governed by PDE from observed data. 

% However, in many practical cases such as floods in urban area, the boundary condition, inputs and dynamics can be very complex such that we can hardly find a feasible mesh free solution.

In the second class, Deep Learning techniques help boost PDE solvers. As one of the earliest trial in this field, \cite{tompson2017accelerating, Tompson2017AcceleratingEF} replaced the time consuming part of the solver to Navier-Stokes Equation, the pressure projector, with a Convolutional Neural Network(CNN)\cite{lecun1998gradient}. More agrressive methods replace entire PDE based solver with a Deep Neural Network\cite{thuerey2018well}. \cite{Wiewel2018LatentspacePT} combined Autoencoder with Long Short Term Memory(LSTM) to learn the temporal evolution of fluid flow. \cite{Kim2018DeepFA} extends the work of \cite{Wiewel2018LatentspacePT} to create a framework for learning data-driven PDE models, and applies it to a smoke simulation problem. Generative Adversarial Neural networks(GANs)\cite{goodfellow2014generative,mirza2014conditional} is applied to achieve super resolution solutions of the regression task\cite{xie2018tempogan}. \kun{There are ome papers by ETH about the lagrangian simulation of PDE.}

% Several exporations about deep learning and physics focuses on the prediction of a Lagrangian system. \cite{battaglia2016interaction} introduces a neural network structure that predicts the 
% In contrast, our work applies deep learning techniques to study the temporal evolution of flood with a large scale realistic setting. We derived an ensemble method to combine two methods to improve the precision, leveraging methods used previously in estimation. Furthermore, we validate the performance of our learned methods, and demonstrate their robustness and their suitability to the measurement update step in estimation algorithms.

% [\cite{Wiewel2018LatentspacePT}] employs CNN and LSTM to learn the discrete solution of a Navier Stokes(check again) equation in some given settings. Convolutional encoder and decoder maps the high dimensional discrete states to a latent space. The LSTM algorithm is employed to learn how the latent space states propogate along time. 

% [well, how accurate it is] employs CNN to map from input information which includes boudary condition and initial condition to states after several time steps. [citation: Deep Fluids: A Generative Network for Parameterized Fluid Simulations]......

% It's worth notice that meshed free method faces problems of high dimensional input and outputs(curse of dimension). We need to reasonably reduce the dimension and find a reasonable learning architecture to avoid overfitting. However, the advantage of mesh based method is that it seems to be able to deal with more complex internal conditions and dynamics. 

% [Well, how accurate is it? A Study of Deep Learning Methods for
% Reynolds-Averaged Navier-Stokes Simulations] and [citation:] are new progresses recently using deep learning architectures to directly learn discrete solutions of partial differential equations. The disadvantage of this model is that it takes $80k$ iterations to train the model. Combined with their deep CNN network and the 128*128 grids, the training cost will be extremely high.\\

% What's more, if we change to a totally different settings, (such as real world topography of floods), the model would need to be trained totally again. Thus, we are thinking about an algorithm efficient in training while reaches the precision needed to predict flood.

% [citation: Deep Fluids: A Generative Network for Parameterized Fluid Simulations] Using Generative 

